Volumetric density measurement in buoyant plumes using Tomographic Background Oriented Schlieren (TBOS)

Buoyant plumes are encountered in both natural and artificial scenarios, ranging from volcanic ash clouds and wildfires to smoke from chimneys and industrial pollutant discharge to rivers and lakes. These plumes are driven by the buoyancy forces arising from the density differences between the plume and the ambient fluids. Measurements of three dimensional density field is limited in literature and not available for buoyant plumes. Such data can lead to better understanding of the pollutant dispersion as well as fundamental nature of concentration dispersion in three-dimensional and turbulent flow. We present the three-dimensional density field measurement in buoyant plumes, particularly for forced and lazy plumes, using an in-house developed experimental rig and associated processing software. The density field reconstruction has been obtained using the tomographic background-oriented Schlieren (TBOS) technique. The experimental rig consists of eight cameras, facing random dot backgrounds placed diametrically opposite, mounted circumferentially around the buoyant plume. For the dot displacement calculation, we use a cross-correlation method. A finite difference-based Poisson solver is employed to calculate projected integrated density. The reconstruction has been performed using the Simultaneous Algebraic Reconstruction Technique (SART). The three-dimensional density field data, thus obtained is validated using existing theoretical models in the literature. We demonstrate that the 3D density field can serve as valuable data for validating and improving theoretical models of plume dynamics e.g. for the lazy plumes the measured density field is effectively used to show the puffing phenomenon.

==> sections/intro.tex <==
\section{Introduction}\label{sec1}
Fluid flows with density variations are prevalent in various natural and industrial applications, including compressible flows, mixing processes, buoyant plumes, and thermals. In many transport processes, the motion of fluid is driven by the interaction of density differences with the gravity field. Buoyancy effects in fluid flows arise from variations in composition or phase, such as those found in ocean circulations or mixtures of liquid and vapor in steam generators. These buoyancy-induced flows often occur on a large scale and over long duration, resulting in turbulent flow mechanisms. For example, plumes are a prominent feature of the steady-state thermal convection in the mantle during volcanic eruptions. Accurate density measurement is essential for effectively modeling and controlling these complex flows. Understanding the intimate details of such flows, including instabilities and transport rates, begins with effective flow visualization technique. Conventional schlieren and shadowgraph imaging methods capture light ray deflection due to refractive index gradients, providing a qualitative view of density changes. The resulting images show deflection patterns compared to a reference image, visually representing density variations. However, this qualitative method does not directly provide detailed flow field information.

Background-Oriented Schlieren (BOS) is a well-established flow visualization technique for measuring density in transparent media, leveraging the relationship between density gradients and refractive index described by the Gladstone-Dale relation \( n-1 = \rho \cdot G\). This non-intrusive method's ability to extract quantitative data has made BOS a widely used optical flow diagnostic tool. First introduced in 1999 by Meier \cite{Meier1998NewOT}, BOS principles have been applied in experimental aerodynamics to extract density fields of vortices generated by helicopter, supersonic jets and more \cite{raffel2000applicability, dalziel2000whole, richard2001principle, 10.1007/978-3-662-08263-8_9}. Tomographic Background-Oriented Schlieren (TBOS) is a variant of BOS that combines tomography with BOS measurements, enabling the measurement of three-dimensional (3D) non-uniform density fields. Tomographic BOS extends the capabilities of BOS by using the apparent deflection of a background pattern from multiple projection angles, allowing for the reconstruction of the instantaneous three-dimensional density field through tomographic algorithms. The first demonstration of tomographic BOS was reported  by Atcheson et al. \cite{atcheson2008time} to estimate the density of an unsteady gas flow. Since then, multi-camera BOS setups have been widely used to reconstruct the instantaneous density distributions in natural convection flows \cite{li2023quantitative}, supersonic jets and heated jets\cite{venkatakrishnan2005density, amjad2023three}. Although many tomographic BOS studies have been investigating the density objects of flames/plumes \cite{grauer2018instantaneous, bathel2019development,liu2020time, liu2021volumetric, hu2023background}, very few literatures are available on the reconstruction of bouyancy driven non-axisymmetric helium plume \cite{bathel2019development}. This study addresses this gap by focusing on the reconstruction of such plumes using TBOS, contributing new insights to this under-explored area.

3D reconstruction in TBOS leverages a variety of algorithms from multiple disciplines, including computed tomography (CT). These algorithms are broadly categorized into analytical and iterative methods based on their solving approaches. The selection of reconstruction algorithms depends on specific requirements. For instance, in the case of axisymmetric flowfields, analytical methods such as the Abel transform, Filtered Back Projection (FBP), and the Analytical Fourier Transform (AFH) are commonly used \cite{venkatakrishnan2005density,tan2015measurement, ohno2018reconstruction}. For non-axisymmetric flowfields, iterative algorithms like the Algebraic Reconstruction Technique (ART), the Simultaneous Iterative Reconstruction Technique (SIRT) and Conjugate Gradient Least Squares (CGLS) are often preferred due to their ability to handle fewer projection angles and noisy data, as well as their flexibility in incorporating prior knowledge during reconstruction \cite{wu2024non, li2024three, atcheson2008time}.

The quality of reconstructed data in TBOS is determined by the reconstruction algorithm. Venkatakrishnan and Meier \cite{venkatakrishnan2004density} reported the first implementation of FBP optical tomography in one plane to  obtain distribution of density field for axisymmetric supersonic flow. However, FBP, a traditional analytical tomographic reconstruction technique based on the Fourier slice theorem, faces challenges in achieving accurate reconstructions with limited projection data. Studies conducted by Goldhahn et al.\cite{goldhahn2007background}, Schröder et al. \cite{schroder2009measurements} and Hartmann et al. \cite{hartmann2016combining} highlighted the shortcomings of FBP in relation to TBOS. Although FBP is orders of magnitude faster than equivalent iterative reconstructions, these studies consistently observed reconstruction artifacts around the test subject due to an inadequate number of views and measurement noise. Further, the studies involving non-axisymmetric applications of TBOS have shown the superiority of the iterative reconstruction techniques as opposed to the analytical ones.

In contrast, Algebraic Reconstruction Techniques (ART), which are iterative, offer improved reconstruction accuracy under conditions of limited projection angles and noisy data \cite{kak2001principles}. ART showed reduced RMS error and peak error in the reconstruction of the turbulent jet and outperformed both FBP and FBP-ART combination, capturing details of the flow \cite{amjad2020assessment}. In this study, the Simultaneous Iterative Reconstruction Technique (SIRT), a variant of ART, has been employed in developing an in-house code to reconstruct the instantaneous density field from BOS measurements. 

The image processing algorithm being used for the estimation of per-pixel displacements between images in the presence and absence of a non-homogeneous medium also affects the quality of reconstructed data. Earlier studies focused on implementing window-based cross-correlation algorithms to extract density information \cite{raffel2018particle}. However, these algorithms suffer from lower spatial resolution, which can be circumvented by using computer vision's optical flow algorithms. Atcheson et al. \cite{atcheson2009evaluation} investigated the application and performance of optical flow-based algorithms such as Lucas-Kanade \cite{lucas1981iterative} and Horn-Schunck \cite{HORN1981185}, in relation to Background-Oriented Schlieren (BOS). In BOS, refraction results in the apparent 2D motion of a background pattern between a reference image, \( I(x, y, t) \), and a distorted image, \( I(x + dx, y + dy, t + dt) \), showing correspondence with the optical flow from computer vision. The mathematical model for optical flow involves the brightness constancy equation \( I(x, y, t) = I(x + dx, y + dy, t + dt) \) and the gradient constraint equation \( I_x u + I_y v = -I_t \) \cite{heineck2021background}. Extensive comparisons of image processing algorithms suggested the superiority of the optical flow algorithm over window-based algorithms \cite{cakir2023assessment,liu2015comparison}. In this study, Horn and Schunck optical flow algorithm has been implemented in developing an in-house code to obtain the 2D BOS signal from each camera.

The objective of this study is to extract the density data of the buoyancy driven 
non-axisymmetric Helium plume by implementing the TBOS. This study aims to compare the reconstruction results obtained from widely used cross-correlation and Horn-Schunck based optical flow algorithm. The investigations involving comparison of the image processing algorithms in relation to the TBOS has not been conducted yet. The paper is organized as follows: Section \ref{BOS} outlines experimental settings, measurement principle of TBOS, image processing algorithms and tomographic reconstruction algorithm  used subsequently; Section \ref{results} studies the reconstruction of the buoyant plume focusing on the impact of image processing algorithms on reconstruction, and the physics of buoyant plume are discussed; and Section \ref{conclusion} provides the main conclusions of this study.


==> sections/introPlumeTheo.tex <==
\section{Plume Theoretical Background}

Can introduce the coordinate system,
major forces
MTT and power law solution

==> sections/methodologyCopyTemp.tex <==

\section{Methodology}\label{sec:methodology}
In this section, we describe our experimental rig, including the buoyant plume generation setup and Background-Oriented Schlieren (BOS) camera arrangements (Sect.~\ref{subsec:meth_bosCamArrangement}). Using this experimental rig, we obtain the raw images of the background with and without plume and process them using our in-house software suite to obtain the volumetric density field. The workflow is described in Sect.~\ref{subSec:dataWorkflow}. 

\subsection{Buoyant plume generation and characterization}\label{subsec:setupPlumGen}
We describe the buoyant plume experimental rig in two parts: the apparatus used to generate a desired buoyant plume and the TBOS  camera setup. 

\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth]{./figures/plumeExpSetUp.eps}
\caption{Schematic of experimental setup for generating buoyant plumes.}%[verify dimensions]}
\label{fig:plumeSetup} 
\end{figure}


The experimental setup for the generation of the buoyant plume is shown schematically in Fig.~\ref{fig:plumeSetup}. Two mass flow controllers, MFC 1 and MFC 2 (Alicat Scientific, MFC-100 slpm, MFC-1000 slpm), are used to precisely intake the dry helium (He) and air gases, which are being supplied from the compressed gas cylinders. Inside a specially designed mixing chamber fitted with silencers \citep{Bharadwaj_Das_2017}, two gases are mixed, then fed to the vertically mounted settling chamber. The settling chamber has a sponge layer and a honeycomb structure that helps to damp out any remaining flow disturbances and to straighten the flow. The He-Air mixture finally passes through a pipe nozzle (exit diameter $D$ = 35 and length 314 mm) with a bell-mouth shaped inlet (diameter 2D)  for smoother entry of plume fluid and discharges into the ambient air. The exit of the nozzle is fixed to a heavy steel bench platform. For further details of plume generation setup, refer to \citep{Bharadwaj_Das_2017}; however, the current setup does not include the seeding mechanism as the seeding is not required. The cuboid acrylic enclosure has also been removed for the ease of installing cameras and background patterns around the setup as described in Fig.~\ref{fig:bosSetUp}. Experiments are performed in a quiet room. 

Given the flow rates $Q_{\text{He}}$ (slpm) and $Q_{\text{Air}}$ (slpm), taking the constant temperature and pressure during mixing, the equivalent source volume flow rate $Q_0 = Q_{\text{He}} + Q_{\text{Air}}$, and the equivalent mass flow rate $m_0 = \rho_{\text{He}} Q_{\text{He}} + \rho_{\text{Air}} Q_{\text{Air}}$ are calculated. The reference properties of pure He and air gases taken for the analysis are presented in Table~\ref{tab:gasRefParams}. Further, the equivalent density of the mixture gas is given as $\rho_0 = m_0/Q_0$. The equivalent dynamic viscosity, $\mu_0$ of the mixture is calculated using Wilke's formula \citep{wilke1950viscosity}. The exit velocity at source, $V_0 =Q_0/\pi b_0^2$, where $b_0=D/2$ is the source radius. The buoyant plumes are characterised using the parameters in Table~\ref{tab:cases}.


\begin{table}[h]
\caption{Properties of helium (He) and air used in the analysis}\label{tab:gasRefParams}%
\begin{tabular}{@{}lll@{}}
\toprule
Property & He  & Air \\
\midrule
density ($\rho$), kg/m$^3$   & 0.1635   & 1.184   \\
dynamic viscosity ($\mu$), Pa$\cdot$s     & 1.984e-5  & 1.849e-5   \\
molecular weight ($m_w$), g/mol       & 4.0026   & 28.966   \\
Gladstone-Dale constant ($G$)\footnotemark[1], m$^3$/kg    & 1.960e-04 & 2.239e-4 \\
\botrule
\end{tabular}
\footnotetext{Experiments were conducted at 298 K temperature and 1 atm pressure.}
\footnotetext[1]{Data from \cite{merzkirch2012flow}.}
\end{table}



\begin{table*}[h]
\caption{Characterization of the buoyant plumes at source (denoted by subscript `0').}
\label{tab:cases}
\centering
\begin{tabular}{@{}p{0.06\textwidth} p{0.025\textwidth} p{0.025\textwidth} p{0.025\textwidth} p{0.025\textwidth} p{0.03\textwidth} cccccc@{}}
\toprule
Release & \multicolumn{2}{c}{$\dot{Q}$ (slpm)} & $Y_{\text{He}}$ & $Y_{\text{Air}}$ & $\rho_0$ & $V_0 $ & $S_0$ & $Re_0$ & $Fr_0$ & $Ri_0$ & $\Gamma_0 \, $ \\
\cmidrule(lr){2-3} 
     & He & Air & & & $\frac{kg}{ m^{3}}$ & $\frac{m}{s}$ & & & & &  \\
\midrule
I & 20 & 10 & 0.22 & 0.78 & 0.50 & 0.52 & 0.43 & 449 & 0.89 & 1.72 & 3.12 \\
II & 20 & 15 & 0.16 & 0.84 & 0.60 & 0.61 & 0.51 & 633 & 1.03 & 0.91 & 1.97 \\
III & 30 & 10 & 0.29 & 0.71 & 0.42 & 0.69 & 0.35 & 494 & 1.18 & 1.31 & 1.98 \\
\botrule
\end{tabular}
\end{table*}


The parameters given in Table~\ref{tab:cases} are the mass fractions $Y$, density ratio $S=\rho_0 / \rho_{\infty}$, Reynolds number $Re=\rho_0 V_0 D/ \mu_{0}$, Froude number $Fr=V_0/ \sqrt{gD}$, and Richardson number $Ri=(\rho_0 - \rho_{\infty}) g D / \rho_{0} V_{0} ^2$. The symbols $\rho_0$, $\rho_{\infty}$, $V_0$, and $D$ denote the density of source, the density of ambient air, velocity at source, and diameter at source, respectively.  The flux balance parameter or the plume function \citep{morton1973scale, hunt2011classical} defined for the finite area source plume $\Gamma_0$ is calculated as $(5 B_0 Q_0^2)/(8 \alpha \sqrt{\pi} M_0^{5/2})$ , where $B_0$ is the source buoyancy flux, $ Q_0 $ is the volume flux, $ M_0$ is the momentum flux, and $ \alpha $ = 0.091 (for Gaussian profiles, \cite{ciriello2020analytical}) is the entrainment coefficient. Based on the source plume function $\Gamma_0$ plume can be characterised \citep{hunt2011classical} to be forced ($0<\Gamma_0<1$), pure ($\Gamma_0 =1$), and lazy ($1< \Gamma_0$). 

A relation between density ($\rho$) and the refractive index ($n$) of the He-Air mixture can be derived \citep{qin2002effect,Ghazwani2016, wanstall2020implications, hu2024reconstruction} using the Gladstone–Dale relation along with the ideal gas law for mixtures, given as:   
\begin{align}
 \label{eq:gladstone-combined}
n - 1 &= \frac{P}{R_u T} \left( G_{\text{He}} \, m_{\text{wHe}} \, \chi_{\text{He}} + G_{\text{Air}} \, m_{\text{wAir}} \,\chi_{\text{Air}} \right) \\
\rho &=  \frac{P m_w}{R_u T} \\
m_w &= m_{\text{wHe}} \, \chi_{\text{He}} + m_{\text{wAir}} \, \chi_{\text{Air}} \\
1 &= \chi _ {\text{He}} + \chi_{\text{Air}}  ;
\end{align}

where $P$, $R_u$, and $T$ denote the pressure, universal gas constant, and temperature, respectively. $G$, $m_w$, and $\chi$ denote the Gladstone–Dale constant, molecular weight, and molar fraction. The subscripts indicate whether the quantity pertains to helium (He) or air. The values of $G$ and $m_w$ are taken from Table~\ref{tab:gasRefParams}. The final relation between the mixture density gradient and the mixture refractive index gradient can be obtained by eliminating $\chi$, resulting in: 

\begin{equation}
\nabla \rho = \left(\frac{ G_{\text{He}} m_{\text{wHe}} - G_{\text{Air}} m_{\text{wAir}} }{m_{\text{wHe}} -  m_{\text{wAir}}} \right)^{-1} \nabla n.
\end{equation}

Using the respective values of He and Air parameters, the equivalent Gladstone-Dale constant for the mixture of He-Air is obtained as 2.2837 $\times 10^{-4}$ m$^3$/kg.

\subsection{Identification of puffing and non-puffing cases}\label{subsec:meth_idPuffNonPuff}
Using the neutral curves for buoyant plume stability from the global stability analysis in \citet{Bharadwaj_Das_2017}, we classify the three release cases in the present study as either laminar or puffing. Puffing buoyant plumes are characterised by the periodic formation of toroidal vortices near the source, which convect downstream. These structures are also responsible for flame flicker and pinch-off in candle flames~\citep{maxworthy1999flickering,xia2018vortex}.

In Fig.~\ref{fig:neutralCurve}, the three solid curves correspond to the density ratios ($S$) of the release cases listed in Table~\ref{tab:cases}. The Reynolds number ($Re$) and Froude number ($Fr$) for each case are plotted. A case is considered stable (laminar) if the point lies to the left of its corresponding neutral curve, and unstable (puffing) if it lies to the right. Furthermore, the farther a point lies from the neutral curve, the stronger the degree of stability or instability it represents. Based on this classification, one case (Release-II) is identified as laminar-non puffing, while the other two (Releases-I and III) are unstable and exhibit puffing behaviour, as seen in Fig.~\ref{fig:neutralCurve}. Release-I lies close to the neutral curve, suggesting it is near the transition between laminar and puffing regimes. In contrast, Release-III lies farther to the right of its stability curve, indicating a higher degree of instability and, hence, stronger puffing behaviour compared to Release-I. These stability characteristics will be referenced in the results section to validate our volumetric density field measurements.

\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth]{./figures/neutralCurves.eps}
\caption{Classifying three plume releases into laminar or puffing regimes using the non-dimensional parametric space of Re-Fr. Solid curves taken from \citep{Bharadwaj_Das_2017} are the neutral stability curves of the primary mode obtained from the global instability analysis and separate the laminar (stable) and puffing (unstable)regions.}
\label{fig:neutralCurve} 
\end{figure}

\subsection{BOS camera arrangement}\label{subsec:meth_bosCamArrangement}
Figure \ref{fig:bosSetUp} depicts the schematic of the camera arrangement for tomographic BOS measurement of the buoyant plume. Eight IMPERX GEV-B2320M-TC000 cameras (2352 x 1768 px) with 85 mm lenses, each facing a background pattern, are placed on a circle around the buoyant plume in such a way that the line-of-sight of the camera and background passes through the centre of the measurement volume. The radius of the circle and angular spacing are 600 mm and $22.5^{\circ}$, respectively.




The background patterns are illuminated using a single, stable high-power (40 W) continuous LED light source that emits in the visible spectrum, with a color temperature of approximately 6500 K (daylight white) and a 1000 W halogen lamp with a color temperature range around 3400 K. It is mounted on the camera side of the rig, positioned sufficiently high above the measurement domain such that the quasi-shadowgraph effects \citep{schmidt2025twenty} caused by the illumination light passing through the phased object are negligible. The details for the assessment of the quasi-shadowgraph effects are presented in Appendix%~\ref{app:quasiShadowEffects}. 

All eight cameras are synchronized using a hardware trigger signal obtained from BNC Model 575 digital/delay pulse generator at 10 fps for Release-I and II and 21 fps for Release-III, with an exposure time of 100~$\mu s$ for acquiring the images simultaneously. The acquisition and processing were performed using a Dell Precision Tower 7810 equipped with an Intel(R) Xeon(R) CPU E5-2650 v3, 2.30GHz (10 cores), 64.0 GB of RAM, and an NVIDIA Quadro K5000 (4 GB) graphics card, running on a 64-bit Windows 10 Pro operating system. The cameras, operating on the GigE Vision protocol, were connected using CAT6 Ethernet cables to two dedicated Network Interface Cards (NICs), with each NIC handling four cameras. The camera control and image acquisition were managed using Bobcat GEV Software and IMPERX ToolKit.  
\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\textwidth]{./figures/plumeExpSetupCombined.png}
\caption{8-camera laboratory setup for Tomographic BOS, centred around the plume: (a) schematic and (b) actual experimental setup.}
\label{fig:bosSetUp} 
\end{figure*} 


\subsection{Data Processing work-flow}
\label{subSec:dataWorkflow}
The raw images obtained from the BOS experimental rig, both in the presence and absence of plumes (i.e., density gradients), are shown in the left part of Fig.~\ref{fig:workflow}. These images, captured from each of the eight cameras, are subjected to further processing. In step one, the ray deflection is computed using a cross-correlation-based approach, resulting in a 2D line-integrated density gradient, typically referred to as projection data in tomographic literature. The obtained data are further subjected to Poisson integration in step two, yielding a line-integrated density. Finally, in step three, tomographic reconstruction is performed using the Simultaneous Algebraic Reconstruction Technique (SART). For the SART reconstruction, one row of data from each of the 2D line-integrated density projections, obtained from each of the eight camera views, is used to form a sinogram. A sinogram is a two-dimensional representation of the projection data for a particular plane. The sinogram is then used as input to the SART algorithm to compute the density field in the plane under consideration. All the density planes are subsequently stacked to form a three-dimensional density field. The data processing workflow is illustrated in Fig.~\ref{fig:workflow}, and the details of each of the three steps are presented in the following sections.  

\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\textwidth]{./figures/workFlow.png}
\caption{Data processing chain of the developed TBOS system }
\label{fig:workflow}
\end{figure*}

\subsubsection{Ray deflection estimation using cross-correlation}\label{subsec:xCorr}
The ray deflection magnitudes obtained from processing the BOS images using the cross-correlation algorithm as detailed in Appendix~\ref{appB:crossCorr}, for all eight cameras, for Release-I and frame-3, are shown in Fig.~\ref{fig:denGrad}. 

\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\textwidth]{./figures/He20Air10NewSnap3Demo8CamRayDeflec.eps}
\caption{Projected density gradient (represented by contour levels) from 8-cameras at the location of background patterns.}
\label{fig:denGrad}
\end{figure*}

\subsubsection{Poisson solver to obtain line integrated density field}\label{subsub:PoisnSolver}
A 2D Poisson integration is performed on the deflection field obtained by each camera using an FDM-based, in-house developed Poisson solver. The projected density gradients ($\int \nabla \rho dz$), as given by the Eq.~(\ref{eq:bosFinal}), are obtained by applying cross-correlation to the background images with and without the plume. Our goal in this step of the reconstruction workflow is to obtain the projected density ($\int \rho dz$) using the projected density gradients. To achieve this, we formulate a Poisson problem to solve for the projected density.

Consider the Poisson equation in 3D for a scaler-valued function $ \psi(x, y, z) $, given by:

\begin{equation}
    \nabla^2 \psi = \frac{\partial^2 \psi}{\partial x^2} + \frac{\partial^2 \psi}{\partial y^2} + \frac{\partial^2 \psi}{\partial z^2} = \phi(x, y, z),
\label{eq:poisson}
\end{equation}
where $ \phi(x, y, z) $ represents the source term. This equation is discretized using the finite difference method (FDM) on a 3D Cartesian grid with uniform spacing $ h_1 $, $ h_2 $, and $ h_3 $ in the $ x $-, $ y $-, and $ z $-directions, respectively. For an interior grid point $ (i, j, k) $, the second-order central differences in each spatial direction (7 point stencil with 3 points in each direction) yield the following discretized equation:

\begin{align}
\frac{\psi_{i+1,j,k} - 2\psi_{i,j,k} + \psi_{i-1,j,k}}{h_1^2} + \nonumber \\
\frac{\psi_{i,j+1,k} - 2\psi_{i,j,k} + \psi_{i,j-1,k}}{h_2^2} + \nonumber \\
\frac{\psi_{i,j,k+1} - 2\psi_{i,j,k} + \psi_{i,j,k-1}}{h_3^2} = \phi_{i,j,k}.
\label{eq:discrete_poisson}
\end{align}

The discritized equation, when applied to each grid point (node), results in one equation. All the equations obtained from each node can be rearranged to form a linear system (Eq.~(\ref{eq:linear_system})). In the linear system, unknown $\psi$ values are rearranged to form vector $\underline{\mathbf{\psi}}$ and the matrix $\mathbf{B}$ includes the coefficient of those unknown values. Therefore, Eq.~(\ref{eq:discrete_poisson}) when applied to each internal node results in one row of the linear system,
\begin{equation}
    \mathbf{B} \underline{\mathbf{\psi}} = \underline{\mathbf{\phi}},
    \label{eq:linear_system}
\end{equation}
where $ \mathbf{B} $ is a sparse matrix and $ \underline{\mathbf{\phi}} $ is the vector of source terms. 

To formulate Poisson problem with projected density gradients, the source function vector $\underline{\mathbf{\phi}}$, defined in Eq.~(\ref{eq:poisson}), is calculated  as:
\begin{equation}
\underline{\mathbf{\phi}}  = \frac{\partial \Delta_x}{\partial x} + \frac{\partial \Delta_y}{\partial y}+\frac{\partial \Delta_z}{\partial z},
\end{equation}
where $\Delta_x$ and $\Delta_y$ are calculated using cross- correlation in PIVlab and the gradient in the optical direction is taken as $\Delta_z = 0$. Neumann boundary conditions, $\frac{\partial \psi}{\partial n} = 0 $, are imposed on each face of our solution domain.  Boundary conditions are incorporated into the system by appropriately modifying the matrix $\mathbf{B} $ and the right-hand side vector $ \underline{\mathbf{\phi}} $ of Eq.~(\ref{eq:linear_system}). A Dirichlet boundary condition, $\psi = \psi_{0}$, is later applied (see Sect.~\ref{subSec:3D-Recon}), post the reconstruction step, to  correct the remaining integration constant in the Poisson solution resulting from the exclusive use of Neumann boundary conditions.

We use MATLAB function `[$\mathbf{L},\mathbf{U},\mathbf{P},\mathbf{Q},\mathbf{D}$] = \texttt{lu}($\mathbf{B}$)` to perform a sparse LU decomposition, which factorizes the matrix $ \mathbf{B}$ as:

\begin{equation}
    \mathbf{P} \left( \mathbf{D} \backslash \mathbf{B} \right) \mathbf{Q} = \mathbf{L} \mathbf{U},
\end{equation}
where $\mathbf{L}$ is a lower triangular matrix, $\mathbf{U}$ is an upper triangular matrix, $\mathbf{P}$ and $\mathbf{Q}$ are permutation matrices, and $\mathbf{D}$ is a diagonal scaling matrix that improves the stability and sparsity of the factorization. 

The solution process consists of two steps. First, forward substitution is used to solve for an intermediate vector $\underline{\mathbf{y}} $ in the system $L \underline{\mathbf{y}} = \mathbf{P} \underline{\mathbf{\phi}}$. Then, backward substitution is applied to solve for the final solution $\underline{\mathbf{\psi}}$ in the system $U \underline{\mathbf{\psi}} = \underline{\mathbf{y}}$. By utilizing row scaling via $\mathbf{D}$, the factorization remains sparse and stable, allowing efficient computation for large-scale systems.

\begin{figure*}[h]
\centering
\includegraphics[width=0.95\textwidth]{./figures/He20Air10NewSnap3Demo8CamPoissIntDen.png}
\caption{Poisson-integrated density field (represented by contour levels) from 8-cameras at the location of background patterns.}
\label{fig:lineIntDen}
\end{figure*} 

Two-dimensional (2D) projected density gradients, computed via cross-correlation, are processed using a Poisson solver. Although the solver is described in three dimensions (3D) for generality, a 2D Poisson integration is employed. The solution of the Eq.~(\ref{eq:linear_system}) yields the projected density fields, $\int \rho dz+C$, where $C$ denotes the remaining integration constant, for each of the 8 cameras (Fig.~\ref{fig:lineIntDen}). These results from the Poisson solver are further used to reconstruct  density in each transverse plan, $\rho(x, y)$, using a tomographic reconstruction algorithm, as described in the following sections. These reconstructed planes are then stacked to form full 3D density field, $\rho(x, y, z)$. 

\subsubsection{Sinogram Interpolation}
\label{sub:sinInt}
Sinogram inpaining, or interpolation, has been shown to improve the reconstruction quality \citep{brooks1978new} by eliminating the streak artefacts \citep{kalke2014sinogram} in sparse angle tomography. Various interpolation methods exist, ranging from geometric approaches \citep{bertram2004directional, constantino2008sinogram, li2011strategy} to data-driven techniques, including machine learning and deep learning-based methods \citep{li2019sinogram, yao2024no, bellens2024machine}. 
To improve the accuracy \citep{li2011strategy} of the reconstruction from sparse angle tomographic measurements, the sinogram from eight projection angles is interpolated using cubic spline interpolation, following the approach in \cite{enjilela2019cubic}. The 2D discrete sinogram data was interpolated using Matlab's "interp2" function, which incorporates cubic splines interpolation. After the interpolation, the number of angular views artificially increases from 8 to 15. A representative interpolated sinogram is shown in Fig.~\ref{fig:Sinogrm}. The interpolation introduces synthesized data between experimentally acquired views, effectively presenting the tomographic reconstruction algorithm with 15 projection angles. In this work, reconstruction using 15 angles with the SART algorithm was observed to produce fewer artefacts than using the original eight projection angles. However, it should be noted that the synthesized data introduced through interpolation assumes a smoothly varying density field between adjacent measured angular views. This assumption appears valid, as the plumes studied, though asymmetric, are laminar in nature and are expected to exhibit smoothly varying features across the azimuthal angular spacing of 22.5$^\circ$.

\begin{figure}[h]
\centering
\includegraphics[width=0.48\textwidth]{./figures/demoSng_cas1Snp3Pln10.png}
\caption{Interpolated sinogram showing synthesized data between original measurements at eight angles. Odd-numbered ticks represent experimental data at 22.5$^\circ$ intervals, while even-numbered ticks indicate interpolated values derived from adjacent true measurements.}
\label{fig:Sinogrm}
\end{figure}



\subsubsection{Tomographic Reconstruction using SART} \label{subSec:3D-Recon}

The forward projection model for the tomographic reconstruction process is first defined, followed by the methods used to solve the inverse problem. 
A projection is defined as the line integral of the function f(x,y) along a ray located at a perpendicular distance t from the origin and oriented at an angle $\theta$ (Fig.~\ref{fig:forwardProj}a). Each ray is uniquely defined by parameters- t and $\theta$. For all the points on the ray, t = xcos($\theta$) + ycos(90-$\theta)$. The projection for the ray ($\theta$, t) is defined as $p_{\theta}(t) = \int_{\text{line}(\theta, t)} f(x,y)\, ds$, which can be expressed in the Radon transform form as $\int \int_{\mathbb{R}^2} f(x, y) \, \delta\left( t - (x \cos \theta + y \sin \theta) \right) \, dx \, dy $. Denoting the Radon transform operator corresponding to ray $(\theta,t)$, indexed by i, as $\mathcal{R}_i$, the projection becomes $=\mathcal{R}_i f(x,y)$.


Assuming that the function can be approximated by N basis functions $\phi(x,y)$, such that $f(x,y)=\tilde{f}(x,y)=\sum  _{j=1} ^N f_j \phi_j(x,y)$, where $f_j$ are the coefficients associated with each basis function. Therefore, the Radon transform, in terms of discretized function f(x,y) can be written as $p_i =\mathcal{R}_i \tilde{f}(x,y)$, substituting discrete approximation of $\tilde{f}(x,y)$ yields $=\mathcal{R}_i \sum  _{j=1} ^N f_j \phi_j(x,y)$ $\rightarrow$ $=\sum  _{j=1} ^N \{ \mathcal{R}_i   \phi_j(x,y) \}  f_j $
 $=\sum  _{j=1} ^N a_{ij}  f_j$ where, $a_{ij}$ denotes the scaler obtained by applying operator $\mathcal{R}_i$ on $j^{th}$ basis function $\phi_j(x,y)$. 

The line integral for Radon transform can also be calculated by sum of discrete values of function $\tilde{f}(s_{ip})$ at points $1<p<P$ at  regular intervals $\delta_p$ (Fig.~\ref{fig:forwardProj}a) on the ray inside the domain - $p_i = \sum_{p=1}^{P}  \tilde{f}(s_{ip}) \, \delta_p$ where, the values $\tilde{f}(s_{ip})$ are calculated using the bilinear interpolation of the basis function surrounding the $p^{th}$ point on $i^{th}$ ray. For ease of forming linear system of equation, it is written as a bilinear contribution from all the shape functions- $\tilde{f}(s_{ip})  = \sum _{j=1}^{N} w_{ijp} f_j$, where $w_{ijp}$ is the weight contribution from j$^{\textit{th}}$ basis function $\phi_j$ to the p$^{\textit{th}}$ point on i$^{\textit{th}}$ ray (Fig.~\ref{fig:forwardProj}a). However, only the four basis functions surrounding the point contribute, since the support of each pyramid-shaped basis function is limited to its four neighboring grid nodes (Fig.~\ref{fig:forwardProj}b).

Now, substituting $\tilde{f}(s_{ip})$ in $p_i = \sum_{p=1}^{P}  \tilde{f}(s_{ip}) \, \delta_p$ results: $p_i = \sum_{p=1}^{P}   \sum _{j=1}^{N} w_{ijp} f_j \, \delta_p$ $\rightarrow$
$=  \sum _{j=1}^{N} \left\{ \sum_{p=1}^{P}    w_{ijp}  \, \delta_p \right\} f_j$. 
Comparing this to the $p_i=\sum  _{j=1} ^N a_{ij}  f_j$, the coefficients $a_{ij}$ can be obtained as 

\begin{equation}
a_{ij}=\sum_{p=1}^{P}    w_{ijp}  \, \delta_p
\label{eq:aijDef}
\end{equation}

Therefore, the final linear system representing the forward projection modelling is given by
\begin{equation}
\mathbf{A} \underline{\mathbf{f}} = \underline{\mathbf{p}}
\label{eq:linSystForward}
\end{equation}
where $\mathbf{A} \in \mathbb{R}^{M \times N}$ is the matrix with coefficient $a_{ij}$ given by Eq.~(\ref{eq:aijDef}), $ \underline{\mathbf{f}} \in \mathbb{R}^{N \times 1}$ is the vector of unknowns or the solution vector, and $\underline{\mathbf{p}} \in \mathbb{R}^{M \times 1}$ is the projection vector obtained by vectorizing the sinogram of the plane under reconstruction. Whereas, the sinogram is formed by extracting the projection data rows, corresponding to plane under consideration, from the solution of Eq.~(\ref{eq:linear_system}), $\underline{\mathbf{\psi}}$. This inverse problem (Eq.~(\ref{eq:linSystForward})) will be solved using Kaczmarz methods of solving algebraic equations \citep{kaczmarz1937, kak2001principles}.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{./figures/forwardProjModel.eps}
\caption{Forward Projection Modelling (a) Radon Transform schematic and (b) The Pyramid shape bilinear basis function of height 1 with support till the  adjacent 4 nodes }
\label{fig:forwardProj} 
\end{figure}

During the implementation, the coefficients $a_{ij}$ of the matrix $\mathbf{A}$ are computed using $\delta_p = \delta / 8$, where $\delta = \mathrm{domSize}~(=48.51~\mathrm{mm}) / \mathrm{nPixRecon}~(=110)=0.44~\mathrm{mm}$. Here, $\mathrm{domSize}$ and $\mathrm{nPixRecon}$ refer to the side length of the reconstruction square and the number of pixels along each side of the reconstructed image, respectively. The value of $\mathrm{domSize}$ is computed using the maximum field of view along the width, $W_{md} = 68.6~\mathrm{mm}$, as $W_{md} / \sqrt{2}$, as detailed in Appendix~\ref{appC:errorEstimation}, Sect.~\ref{appC:camFOV}, and Fig.~\ref{fig:camFOV}.

The analytical tomographic reconstruction technique such as Filtered Back Projection (FBP) based on the Fourier slice theorem, though providing a faster reconstruction, suffers from reconstruction accuracy when there are fewer projections. On the other hand, the Algebraic reconstruction techniques (ART) which are iterative provide better reconstruction accuracy with limited projection angles and noisy data \citep{kak2001principles}. In this study, the Simultaneous Algebraic Reconstruction Technique (SART), a variant of ART, is employed to develop an in-house code for reconstructing the instantaneous density field using data obtained from BOS measurements. Unlike ART, where the solution $\underline{\mathbf{f}}$ is updated after the consideration of each ray, SART averages the corrections for all the rays and uses the averaged value to update the solution. This completes one iteration, and the process continues until a suitable convergence criterion is met. The iteration step in SART can be mathematically represented as follows:
 
\begin{equation}
 \label{eq:SART_hann}
\underline{\mathbf{f}}^{(k+1)} =\underline{\mathbf{f}}^{(k)} + \frac{1}{M} \sum_{i=1}^{M} \left( \frac{p_i - \underline{\mathbf{a}}_i \cdot\underline{\mathbf{f}}^{(k)}}{\underline{\mathbf{a}}_i \cdot \underline{\mathbf{a}}_i} \right) \underline{\mathbf{t}}_i,
 \end{equation} 
 
where the vector of unknowns at $k^{\textit{th}}$ iteration is $\underline{\mathbf{f}}^{(k)} = [f_1, f_2, \dots, f_N]^T$, $\underline{\mathbf{a}}_i = [a_{i1}, a_{i2}, \dots, a_{iN}]$ represents the $i^{\text{th}}$ row of the matrix $ \mathbf{A} $ with elements $a_{ij}$, and $\underline{\mathbf{t}}_i = [t_{i1}, t_{i2}, \dots, t_{iN}]$ is the $i^{\text{th}}$ row of the matrix with elements $t_{ij}$. $N$ is the total number of unknowns or grid points, and $M$ is the total number of projection rays. The initial guess for the solution vector $\underline{\mathbf{f}}^{(0)}$is set to $\underline{\mathbf{0}}$. 


The elements $t_{ij}$ are calculated as:
 \begin{equation}
t_{ij}=\sum_{p=1}^{P} h_{ip} \,    w_{ijp}  \, \delta_p,
\label{eq:tijDef}
\end{equation}
where $h_{ip}$, for $1 < p < P$, is the Hanning window applied along the ray $i$ over $P$ discrete points.  The hanning window along each projection ray, similar to Hamming window that was found to give superior results \citep{andersen1984simultaneous, kak2001principles}, has been employed.

In the Simultaneous Algebraic Reconstruction Technique (SART), the iterative reconstruction process is terminated when the relative percentage change in the solution vector norm falls below a predefined threshold, $\epsilon = 4\%$. The stopping criterion is defined as $\|\underline{\mathbf{f}}^{(k)} -\underline{\mathbf{f}}^{(k-1)}\|_2 \, / \, \|\underline{\mathbf{f}}^{(k)}\|_2  \times 100 < \epsilon$, where $\underline{\mathbf{f}}^{(k)} $ and $\underline{\mathbf{f}}^{(k-1)} $ represent the current and previous solution vectors, respectively, and $\|\cdot\|_2$ denotes the Euclidean norm (i.e., $\|\underline{\mathbf{f}}\|_2 = \sqrt{\sum_{i=1}^n f_i^2}$). The threshold $\epsilon = 4\%$ was empirically chosen using multiple trials on the reconstruction quality for physical consistency such as centre line Gaussian profiles, necking of the lazy plume, and the convection of the structures. This criterion monitors the stability of the solution vector, which represents the reconstructed image, ensuring convergence while preventing over-iteration that could amplify noise \citep{andersen1984simultaneous, warnett2025don}. Though, a more formal, quantitative method for determining the optimal stopping point may further improve reconstruction accuracy. In the future, probably L-curve \citep{hansen1992analysis} or any other suitable method \citep{hansen2010discrete} will be used. Though typically used for explicitly regularized inversions, the L-curve method can be used for unregulated iterative inversions also, where the number of iterations play the role of regularization parameter \citep{hansen2010discrete}.

After the reconstruction, the axis grids- x,y, and z are scaled down to the scaling factor (mm/pixel) of measurement domain which is half of the scaling factor at the background level. Furthermore, the density field is post-processed to correct the undetermined integration constant due to the use of all Neumann boundary conditions in the Poisson integration step as described in Sect.~\ref{subsub:PoisnSolver}. Using all Neumann boundary conditions a smoother transition in the solution is obtained. A Dirichlet boundary condition with source density $\rho_0$ for each case at the first reconstruction plane at the nozzle exit is used to correct for the integration constant. Next, values outside the circular region (shown by dashed red circle in Fig.~\ref{fig:forwardProj}) ($x^2 + y^2 \leq (L/2)^2$, $L$ being the square domain size) were set to $\rho_{\text{air}}$ to remove the noise in the corners of the reconstruction domain. Also, values where $\rho > \rho_{\text{air}}$ are set to $\rho_{\text{air}}$ to enforce the physical constraint, however such values were found only near the circumference of the circle defined above. Finally, a 3D smoothing filter is applied using MATLAB’s \texttt{smooth3} function \citep{MATLAB:smooth3} with the `box' method which performs a moving average over each cubical window of size 5x5x5 grids, reducing the high frequency noise. A detailed discussion on the effect of each post processing step defined here is presented in Appendix~\ref{append:D} and Fig.~\ref{fig:sngInterpAndPostProcessing}.

A representative post-processed instantaneous reconstructed density plane for Release-III at an arbitrary time instance is shown in Fig.~\ref{fig:denPlaneDemo}.
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{./figures/demoRecon_cas1Snp3Pln10.png}
\caption{A representative instantaneous reconstructed density plane extracted at an arbitrary time instance from the reconstructed density field of Release-I, snap3 at a height of 6.17 mm from source.}
\label{fig:denPlaneDemo}
\end{figure} 
